Constraints on the galaxy "main sequence" at z>5: the stellar mass of HDF850.1

We present rest-frame optical and near-infrared detections of one of the highest redshift submm-selected galaxies to date, HDF850.1. We do not detect the previously proposed counterpart HDF850.1K in new deep J and H-band HST WFC3 data, placing a strong limit of H-K>3.8, concluding that the K-band source is spurious. However, we detect 5.8um and 8um emission co-located with the submm in deblended images. After modelling and removing the flux contributions from another foreground galaxy, we constrain the stellar mass of HDF850.1 to be (2.5+/-1)x10^{11} Msun/mu for a lensing magnification mu=1.9+/-0.3, with a specific star formation rate of 8.5 Gyr^{-1}, faster than the 1-4 Gyr^{-1} observed for UV-selected galaxies at this epoch.

==> sed.tex <==
%
\subsection{SED modelling}

We perform the SED fitting analysis on the detected HST sources 3-577.0, 3-586.0 and 3-593.0 (Williams et al. 1996) in order to check by flux subtraction the models emission of HDF850.1 and HDF850.1K in the IRAC 3.6 and 4.5 $\mu$m (??).
To perform the multi-wavelength fitting procedure we adopt the popular \texttt{LePhare} (Arnouts et al. 1999; Ilbert at al. 2006). We use the F300W, F450W, F606W, F814W WFCP2 and J, H, K NICMOS photometry listed in the Fernandez-Soto 1998 catalogue. We then extrapolate from the best fit SED the J and H WFC3 as well as the IRAC 3.6,4.5, 5.8, 8.0 $\mu$m photometry for each source through the convolution between the model and each filter transmission curve.

The sources considered here have already an associated estimate of the redshif: photometric redshift in the case of 3-586.0, 3-593.0 by Fernandez-Soto 1998 and spectroscopic redshift for the 3-577.0 obtained by ???; we can thus perform the fit using the known redshift and then check the reliability of our modelled photometry by being able to reproduce the tabulated redshift estimate from our best fit solution.

As extinction law we adopt the Calzetti at al. 2000 and we use two set of SED to test our method: the SWIRE templates by Polletta et al. 2007 listed in Tab. \ref{sed.list} and the stellar population synthesis model by Bruzual \& Charlot 2003.

The resulting modelled fluxes of the galaxies from the best fit obtained by both the procedure are very similar each other. At any rate, since our task is to obtain a good extrapolation of the J and H WFC3 and IRAC bands for these galaxies and given our pour constraints on the fit at longer wavelengths, we find more reasonable to take as more reliable the best fit obtained with the Polletta et al. 2007 SED since they are based on real observed Spitzer galaxies. The resulting fluxes are reported in the Tab. \ref{fluxes} below.

\begin{table}
\centering
%\begin{tiny}
\begin{tabular}{c|c|c}
\hline
\textbf{Index} & \textbf{SED Class} & \textbf{Spectral Type}\\
\hline\hline
01 & Ell13 & Elliptical\\
02 & Ell5& Elliptical\\
03 & Ell2& Elliptical\\
04 & S0& Spiral\\
05 & Sa& Spiral\\
06 & Sb& Spiral\\
07 & Sc& Spiral \\
08 & Sd& Spiral\\
09 & Sdm& Spiral\\
10 & Spi4& Spiral\\
11 & N6090& Starburst\\
12 & M82& Starburst\\
13 & Arp220& Starburst\\ 
14 & I20551& Starburst\\
15 & I22491& Starburst\\
16 & N6240& Starburst\\
17 & Sey2& Obscured AGN\\
18 & Sey18& Obscured AGN\\
19 & I19254& Obscured AGN\\
20 & QSO2& Unobscured AGN\\
21 & Torus& Unobscured AGN\\
22 & Mrk231& Obscured AGN\\
23 & QSO1& Unobscured AGN\\
24 & BQSO1& Unobscured AGN\\
25 & TQSO1& Unobscured AGN\\
\hline
\end{tabular}
%\end{tiny}
\caption{List of the Polletta et al. 2007 SEDs used to perform the SED fiitting analysis.}
\label{sed.list}
\end{table}
%

\begin{table}
\centering
%\begin{tiny}
\begin{tabular}{c|c|c|c|c|c|c|c}
\hline
\textbf{Source} & \textbf{Redshift} & \textbf{J/WFC3} & \textbf{H/WFC3} & \textbf{3.6 $\mu$m} & \textbf{4.5 $\mu$m} & \textbf{5.8 $\mu$m} & \textbf{8.0 $\mu$m}\\
\hline\hline
3-577.0 & 3.36 & 0.0660 & 0.0911 &   0.2436 & 0.2681 & 0.2669 &  0.2701\\
3-586.0 & 1.22 & 4.0255 & 5.5979 & 10.5980 & 9.4021 & 6.0817 & 4.3015 \\
3-593.0 & 1.76 & 0.3746 & 0.4643 &   0.6059 & 0.5316 & 0.4341 & 0.3084 \\
\hline
\end{tabular}
%\end{tiny}
\caption{Extrapolated fluxes from the best fit SED for each galaxy. The fluxes has to be interpreted as the total flux at each band and are expressed in $\mu$Jy.}
\label{fluxes}
\end{table}

%\begin{figure*}
%\begin{center}
%   {\myincludegraphics{width=0.45\textwidth}{\figdir{}/Hyperz-fit-sb_new.png}}
%   {\myincludegraphics{width=0.45\textwidth}{\figdir{}/Hyperz-fit-sd.png}}
%   {\myincludegraphics{width=0.45\textwidth}{\figdir{}/Hyperz-fit-sdm_new.png}}
%\end{center}
%\caption[Typical \texttt{Hyperz} best fit results]{Typical \texttt{Hyperz} best fit results. The plot shows in red the best fit SED and in black the observed data points. The name of the SED template of best fit is on the right, the subscript \textit{new} stands for the modified templates by \cite{Gruppioni2010}. Above the SED template name is the redshift of the source and redshift flag: 3 stands for photometric, 9 stands for spectroscopic. At the top left one finds the ID of the source, the flux, the SNR and the $\chi^2$  of the SPIRE extraction for the 250, 350 and 500 $\mu$m respectively, then the $\chi^2$ and the probability of the fit given by \texttt{Hyperz}.}
%\label{Hyperz-fit}
%\end{figure*}
%

\clearpage
\newpage

%
\begin{thebibliography}{}
%
% MNRAS-Style
%
\bibitem[\protect\citeauthoryear{Arnouts et al.}{1999}]{Arnouts1999} Arnouts, S., Cristiani, S., Moscardini, L., et al.\ 1999, \mnras, 310, 540 
\bibitem[\protect\citeauthoryear{Bruzual \& Charlot}{2003}]{BC03} Bruzual, G., \& Charlot, S.\ 2003, \mnras, 344, 1000 
\bibitem[\protect\citeauthoryear{Calzetti et al.}{2000}]{Calzetti2000} Calzetti, D., Armus, L., Bohlin, R.~C., et al.\ 2000, \apj, 533, 682 
\bibitem[\protect\citeauthoryear{Fern{\'a}ndez-Soto et al.}{1999}]{Soto1999}Fern{\'a}ndez-Soto, A., Lanzetta, K.~M., \& Yahil, A.\ 1999, \apj, 513, 34 
\bibitem[\protect\citeauthoryear{Ilbert et al.}{2006}]{Ilbert2006} Ilbert, O., Arnouts, S., McCracken, H.~J., et al.\ 2006, \aap, 457, 841 
\bibitem[\protect\citeauthoryear{Polletta et al.}{2007}]{Polletta2007} Polletta M., et al., 2007, ApJ, 663, 81
\bibitem[\protect\citeauthoryear{Williams et al.}{1996}]{Williams1996} Williams, R.~E., Blacker, B., Dickinson, M., et al.\ 1996, \aj, 112, 1335 
\end{thebibliography}
%
\bsp
%
\label{lastpage}
%
\end{document}

